Half-Space Power Diagrams and Discrete Surface Offsets

We present an efficient, trivially parallelizable algorithm to compute offset surfaces of shapes discretized using a dexel data structure. Our algorithm is based on a two-stage sweeping procedure that is simple to implement and efficient, entirely avoiding volumetric distance field computations typical of existing methods. Our construction is based on properties of half-space power diagrams, where each seed is only visible by a half-space, which were never used before for the computation of surface offsets. The primary application of our method is interactive modeling for digital fabrication. Our technique enables a user to interactively process high-resolution models. It is also useful in a plethora of other geometry processing tasks requiring fast, approximate offsets, such as topology optimization, collision detection, and skeleton extraction. We present experimental timings, comparisons with previous approaches, and provide a reference implementation in the supplemental material.

==> figs/tex/three_segments.tex <==
\begin{figure}[htbp!]
	\centering

	\hfill{}
	\includegraphics[width=0.8\linewidth]{figs/img/appendix/three-segments.pdf}
	\hfill{}

	\caption{The example of computing the Voronoi vertex generated by three line segments. The coordinates are $(x,y_i,\zIn_i,\zOut_i)$, i=1,2,3}

	\label{fig:morpho:three-segments}
\end{figure}

